Adapting Foundation Models for Annotation-Efficient Adnexal Mass Segmentation in Cine Images

Adnexal mass evaluation via ultrasound is a challenging clinical task, often hindered by subjective interpretation and significant inter-observer variability. While automated segmentation is a foundational step for quantitative risk assessment, traditional fully supervised convolutional architectures frequently require large amounts of pixel-level annotations and struggle with domain shifts common in medical imaging. In this work, we propose a label-efficient segmentation framework that leverages the robust semantic priors of a pretrained DINOv3 foundational vision transformer backbone. By integrating this backbone with a Dense Prediction Transformer (DPT)-style decoder, our model hierarchically reassembles multi-scale features to combine global semantic representations with fine-grained spatial details. Evaluated on a clinical dataset of 7,777 annotated frames from 112 patients, our method achieves state-of-the-art performance compared to established fully supervised baselines, including U-Net, U-Net++, DeepLabV3, and MAnet. Specifically, we obtain a Dice score of 0.945 and improved boundary adherence, reducing the 95th-percentile Hausdorff Distance by 11.4% relative to the strongest convolutional baseline. Furthermore, we conduct an extensive efficiency analysis demonstrating that our DINOv3-based approach retains significantly higher performance under data starvation regimes, maintaining strong results even when trained on only 25% of the data. These results suggest that leveraging large-scale self-supervised foundations provides a promising and data-efficient solution for medical image segmentation in data-constrained clinical environments. Project Repository: https://github.com/FrancescaFati/MESA

==> sec/5_results.tex <==
\section{Results}

% \begin{table*}[t]
% \centering
% \caption{Comparison across datasets that provide paired diffuse-only ground truth. 
% The best score in each metric is highlighted in \textbf{bold}.}
% \begin{tabular}{l|ccc|ccc|ccc}
% \toprule
%  & \multicolumn{3}{c|}{Lesion} 
%  & \multicolumn{3}{c|}{Fluid} 
%  & \multicolumn{3}{c}{Solid} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
% \textit{Method}
% & DSC$_m\!\downarrow$ & Acc$\uparrow$ & IoU$\uparrow$
% & DSC$_m\!\downarrow$ & Acc$\uparrow$ & IoU$\uparrow$
% & DSC$_m\!\downarrow$ & Acc$\uparrow$ & IoU$\uparrow$ \\
% \midrule
% Unet~\cite{24}
% & 0.006 & \textbf{24.863} & 0.868
% & 0.001 & \textbf{33.815} & 0.982
% & \textbf{0.001} & \textbf{37.318} & \textbf{0.971} \\

% Unet++~\cite{21,20}
% & 0.050 & 14.101 & 0.645
% & 0.089 & 12.009 & 0.604
% & 0.024 & 18.102 & 0.432 \\

% Manet~\cite{2}
% & 0.007 & 23.675 & 0.839
% & 0.005 & 27.386 & 0.961
% & 0.002 & 31.628 & 0.952 \\

% DeepLabv3~\cite{25}
% & 0.007 & 23.786 & 0.838
% & \textbf{0.001} & 32.885 & 0.978
% & 0.001 & 35.857 & 0.963 \\

% \midrule
% OURS
% & \textbf{0.004} & 17.230 & \textbf{0.911}
% & 0.003 & 17.610 & \textbf{0.988}
% & 0.002 & 28.415 & \textbf{0.971} \\
% \bottomrule
% \end{tabular}
% \end{table*}


% \begin{table}[t]
% \centering
% \small
% \setlength{\tabcolsep}{6pt}
% \begin{tabular}{lcccc}
% \toprule
% Method & Dice $\uparrow$ & IoU $\uparrow$ & Sens. $\uparrow$ & Spec. $\uparrow$ \\
% \midrule
% U-Net &  &  &  &  \\
% U-Net++ &  &  &  &  \\
% DeepLabV3 &  &  &  &  \\
% MAnet &  &  &  &  \\
% \midrule
% DenseDINO (ours) &  &  &  &  \\
% \bottomrule
% \end{tabular}
% \caption{Binary adnexal mass segmentation on the test set. Values are mean $\pm$ std across cases.}
% \label{tab:main}
% \end{table}

==> sec/6_discussion.tex <==
\section{Discussion}

==> sec/8_EXTRA.tex <==
\section{Copied and Pasted from SOTA}
\label{sec:intro}
\subsection{Whitney et al 2024 \cite{whitney2024ai}}
Segmentation of ovarian/adnexal masses from surrounding tissue on ultrasound images is a challenging task. The separation of masses into different components may also be important for radiomic feature extraction. Adnexal masses can be found in the ovary, fallopian tube, or surrounding tissue and represent a
heterogeneous spectrum of benign, borderline, and malignant entities. They are common, with
an incidence of 35\% in premenopausal and 17\% in postmenopausal women. Pathologies differ
across age ranges and geographical areas, but most adnexal masses (∼85\%) are benign and
without symptoms. Most can be managed conservatively with a follow-up by clinical exam and
sequential imaging, without surgical intervention. It is estimated that 10\% of all women will be
operated on for an adnexal mass during their lifetime, potentially resulting in peri- and post-
operative morbidity (e.g., infections, injury to adjacent organs, and anesthetic complications).
However, although most adnexal masses are benign, and ovarian cancer is a rare disease with
an incidence of one case per 91 women, it is the most lethal gynecology malignancy, with
a 5-year survival rate of only 30\% when diagnosed in advanced stages.
Ultrasound imaging plays a key role in the evaluation of patients with adnexal masses. It is
noninvasive, widely available, safe, and low cost. Assessments are based mainly on qualitative
features, including mass morphology, margins and echogenicity, the presence of solid elements,
acoustic shadowing, vascular flow signals, and interaction with the surrounding tissues. Given
that ultrasound imaging is used early during the evaluation of any lower abdominal, back, or
flank pain, the incidental detection of adnexal masses has substantially increased. Several
ultrasound-based risk models have been developed to standardize adnexal mass assessment, such
as the International Ovarian Tumor Analysis (IOTA) Simple Rules, the IOTA Assessment of
Different NEoplasias in the adneXa model, and the American College of Radiology Ovarian-
Adnexal Reporting and Data (O-RADS)14 risk stratification system with the goal of reducing
false positive and false negative assessments. Recent studies comparing the performance of the
risk stratification systems in differentiating between benign and malignant adnexal masses in
cohorts in the United States reported strong performance of all models. However, these mod-
els rely on qualitative assessments of the masses, which are subject to inter- and intra-observer
variability, and achieving expertise in ultrasound interpretation takes time to gain and is not
ubiquitously available. Artificial intelligence (AI)-based automation for the assessment of adnexal masses on ultrasound images may provide decision support tools that are more quantitative, more robust, and
better performing than qualitative-based systems. Our long-term goal is to develop an AI-based
pipeline that improves diagnostic accuracy for adnexal masses and decreases unnecessary sur-
geries for asymptomatic benign masses while being efficiently integrated into a clinical work-
flow. The first step is to automatically (i.e., objectively) outline the area of interest, the adnexal
mass. When done manually, segmentations require expertise, are time-consuming, and are prone to errors even when done by experts. Adnexal mass assessments are challenging tasks requiring knowledge and expertise. Thus there is a rising interest in developing computer-aided diagnosis tools to ease and improve sonographic
evaluations, diagnostic accuracy, and patient outcomes. The first and crucial step in a machine
learning pipeline is an accurate outlining of the region of interest, the adnexal mass borders. 
This approach has the potential to improve operational efficiency and clinical workflow as it only requires the clinicians to define a bounding box surrounding the adnexal mass, thus also reducing the variability in manually outlining the region of interest. Several groups have studied the use of the U-Net architecture or its variations for segmentation of areas of interest on medical images across a variety of anatomies and physiologies as well as modalities, including ultrasound, computed tomography, and magnetic resonance imaging of ovarian masses. However, the use of U-net segmentation for adnexal mass assessments on ultrasound has been limited. In addition, most ultrasound-based radiomics classification studies for adnexal masses have used manual segmentation. Recently, Barcroft et al.54 reported a segmentation and classification approach for adnexal masses on ultrasound; they evaluated several DL architectures for the segmentation task,
and their best-reported U-net model resulted in a median Dice score of 0.85 in an external test set
(184 masses) compared to manual expert outlines Our study has some limitations, typical for an investigation of this nature. First, the study was limited to a segmentation task (i.e., segmentation of adnexal masses from the background, followed by internal component segmentation). By design, it did not incorporate a mass detection task or mass classification task, as we are especially interested in segmenting masses based upon
user-provided ROIs around the masses. Ultrasound is also affected by sound wave traits in biological tissue, which can result in speckle noise, artifacts, and acoustic shadowing. All of these factors impact any AI pipeline for ultrasound in medical imaging. All of these factors impact any AI pipeline for ultra-
sound in medical imaging.  

\subsection{Barcroft et al 2024 \cite{barcroft2024machine}}
The poor prognosis of OC is mainly attributed to most women (75\%) presenting late, with advanced stage disease. Unfortunately, an effective OC screening programme does not exist, diagnosis is reliant upon prompt recognition of gynaecological symptoms and accurate interpretation of clinical imaging. Adnexal masses are common, affecting up to 18\% of postmenopausal women in the UK4. The accurate classification of adnexal masses is fundamental to ensure malignant adnexal masses are promptly identified and undergo surgical intervention by an appropriately trained surgeon. Particularly in younger women and those with an asymptomatic lesion, it is important that those with a benign mass are not subjected to unnecessary
intervention, with potential complications. 

\subsection{Liu et al 2025}
The therapeutic approach for malignant and benign adnexal masses is fundamentally distinct. Consequently, precise differentiation between malignant and benign lesions is critical for optimizing patient care. Ultrasound currently stands as the primary imaging modality for adnexal lesions. Considering the diverse morphological features presented by these masses, interpreting ultrasound images can be intricate, with diagnostic accuracy heavily dependent on the radiologist’s experience and subjective assessment. However,
the complexity of the system and the varied presentation of adnexal masses pose a challenge for radiologists, particularly those with less experience. 

\subsection{Li et al 2022}
Adnexal masses are widespread in women. Most masses are benign and some may disappear spontaneously. Conservative management is often advised. However, some adnexal masses classified as borderline or malignant may pose a significant risk. Therefore, the primary diagnosis depends mainly on imaging techniques. MRI provides the best means of evaluating ovarian masses but has low sensitivity for detection of masses [2]. In contrast, ultrasound is considered to be the first-line imaging modality to assess adnexal tumors. Of these various methods, subjective assessment (SA) by expert sonographers remains the most accurate ultrasound imaging diagnostic approach to distinguish between benign and malignant adnexal tumors, but there is a shortage of expert sonographers in clinical work.

\subsection{Lebbos et al 2022 \cite{lebbos2022adnexal}}
Ovarian cancer is the most lethal gynaecological malignancy. The disease is most commonly asymptomatic at its early stages and its diagnosis relies on expert evaluation of transvaginal ultrasound images.
Ultrasound is the first-line imaging modality for characterising adnexal masses, it requires significant expertise and its analysis is subjective and labour-intensive, therefore open to error. Hence, automating processes to facilitate and standardise the evaluation of scans is desired in clinical practice.
Accurate classification of adnexal masses is necessary to reduce incorrect diagnosis and unnecessary surgeries. With an eﬃcient workflow, population screening for ovarian cancer could be feasible, leading to earlier disease detection and increased survival rates. Evidently, there is tangible value in developing a tool able to automatically extract the features in transvaginal ultrasounds accurately and consistently.
A major challenge of ovarian cancer diagnosis is the accurate interpretation of ultrasound images. Although ultrasound is the imaging modality of choice, as it is accessible, non-invasive, and does not use radiation, it is also “notorious for having significant noise with a low signal-to-noise ratio” [18]. This represents a challenge for both medical experts and segmentation algorithms. The wide variety in shape and size of adnexal masses can also pose challenges for segmentation. 
Deep neural networks such as nnU-Net [8] require a large amount of data to perform well. This requirement is commonly addressed with extensive data augmentation techniques such as rotating and scaling.


%-------------------------------------------------------------------------



